Multi-Decoder Networks with Multi-Denoising Inputs for Tumor Segmentation

Automatic segmentation of brain glioma from multimodal MRI scans plays a key role in clinical trials and practice. Unfortunately, manual segmentation is very challenging, time-consuming, costly, and often inaccurate despite human expertise due to the high variance and high uncertainty in the human annotations. In the present work, we develop an end-to-end deep-learning-based segmentation method using a multi-decoder architecture by jointly learning three separate sub-problems using a partly shared encoder. We also propose to apply smoothing methods to the input images to generate denoised versions as additional inputs to the network. The validation performance indicate an improvement when using the proposed method. The proposed method was ranked 2nd in the task of Quantification of Uncertainty in Segmentation in the Brain Tumors in Multimodal Magnetic Resonance Imaging Challenge 2020.

==> 2020 - Minh - Multi-Decoder Networks with Multi-Denoising Inputs for Tumor Segmentation/glossaries.tex <==
\makeglossaries

\newacronym[plural=CNNs,firstplural=Convolutional Neural Networks (CNNs)]{cnn}{CNN}{Convolutional Neural Network}

\newacronym[plural=FCNs,firstplural=Fully Convolutional Networks (FCNs)]{fcn}{FCN}{Fully Convolutional Network}

\newacronym{dl}{DL}{deep learning}
\newacronym{qcmlb}{QC-MLB}{Question-Centric Multimodal Low-rank Bilinear}
\newacronym{bert}{BERT}{Bidirectional Encoder Representations from Transformers}
\newacronym{bleu}{BLEU}{Bilingual Evaluation Understudy}
\newacronym{mlm}{MLM}{Masked Language Model}
\newacronym{nsp}{NSP}{Next Sentence Prediction}
%\newacronym{cv}{CV}{computer vision}
\newacronym{relu}{ReLU}{rectified linear unit}
\newacronym{lrelu}{LeakyReLU}{leaky rectified linear unit}
\newacronym{nn}{NN}{neural network}
\newacronym{chal}{ImageCLEF-VQA-Med}{ImageCLEF-VQA-Med}
\newacronym{proposed}{\textit{\textless~Model~\textgreater}}{\textbf{Full name of the proposed model}}
\newacronym{mri}{MRI}{magnetic resonance imaging}
\newacronym{kits}{KiTS19}{Kidney Tumor Segmentation Challenge 2019}
\newacronym{ibsr}{IBSR18}{Internet Brain Segmentation Repository}
\newacronym{hene}{HeNe}{Ume{\aa} Head and Neck}
\newacronym{pros}{ProST}{Ume{\aa} Prostate}

\newacronym{ct}{CT}{computed tomography}
\newacronym{t1c}{T1c}{post-contrast T1-weighted}
\newacronym{t2}{T2w}{T2-weighted}
\newacronym{t1}{T1w}{T1-weighted}
\newacronym{flair}{FLAIR}{T2  Fluid  Attenuated  Inversion  Recovery}
\newacronym{lgg}{LGG}{low-grade glioma}
\newacronym{hgg}{HGG}{high-grade glioma}

\newacronym{svm}{SVMs}{Support-vector Machines}
\newacronym{crf}{CRF}{Conditional Random Field}
\newacronym{vae}{VAE}{Variational Auto-Encoder}
\newacronym{tunet}{TuNet}{End-to-end Hierarchical Tumor Segmentation using Cascaded Networks}
\newacronym{dram}{DRAM}{dynamic random access memory}
% \newacronym{gpu}{GPU}{graphics processing unit}
% \newacronym{gpus}{GPUs}{graphics processing units}
\newacronym[plural=GPUs,firstplural=graphics processing units (GPUs)]{gpu}{GPU}{graphics processing unit}

\newacronym{hpc2n}{HPC2N}{High Performance Computer Center North}

\newacronym{snic}{SNIC}{Swedish National Infrastructure for Computing}

\newacronym{dsc}{DSC}{S{\o}rensen-Dice coefficient}
\newacronym{se}{SE}{standard error}
\newacronym{seb}{SEB}{Squeeze-and-Excitation block}
\newacronym[plural=REBs,firstplural=ResNet blocks]{res}{REB}{ResNet block}
\newacronym{hd}{HD}{Hausdorff distance}
\newacronym{hd95}{HD95}{$95^{th}$ percentile of the Hausdorff distance}
\newacronym{dauc}{DAUC}{Dice Area Under Curve}
\newacronym{rftp}{RFTPs}{Ratio of Filtered True Positives}
\newacronym{rftn}{RFTNs}{Ratio of Filtered True Negatives}

\newacronym[plural=SDs,firstplural=standard deviations (SDs)]{sd}{SD}{standard deviation}
\newacronym{brats}{BraTS 2020}{Brain Tumors in Multimodal Magnetic Resonance Imaging Challenge 2020}


\newacronym{mdnet}{MDNet}{End-to-end Multi-Decoder Cascaded Network for Tumor Segmentation}
\newacronym{ce}{CE}{categorical cross--entropy}

\newacronym{miccai}{MICCAI}{International Conference on Medical Image Computing and Computer Assisted Intervention}
